Optimal Auctions with Convex Perceived Payments

Myerson derived a simple and elegant solution to the single-parameter revenue-maximization problem in his seminal work on optimal auction design assuming the usual model of quasi-linear utilities. In this paper, we consider a slight generalization of this usual model---from linear to convex "perceived" payments. This more general problem does not appear to admit a solution as simple and elegant as Myerson's. While some of Myerson's results extend to our setting, like his payment formula (suitably adjusted), others do not. For example, we observe that the solutions to the Bayesian and the robust (i.e., non-Bayesian) optimal auction design problems in the convex perceived payment setting do not coincide like they do in the case of linear payments. We therefore study the two problems in turn. We derive an upper and a heuristic lower bound on expected revenue in our setting. These bounds are easily computed pointwise, and yield monotonic allocation rules, so can be supported by Myerson payments (suitably adjusted). In this way, our bounds yield heuristics that approximate the optimal robust auction, assuming convex perceived payments. We close with experiments, the final set of which massages the output of one of the closed-form heuristics for the robust problem into an extremely fast, near-optimal heuristic solution to the Bayesian optimal auction design problem.

==> programs/mpdesc_brm_xa_rel_lim.tex <==

\subsubsection{BRM, Ex-ante Relaxation (Truncated)}
\label{sssec:mpdesc_brm_xa_rel_lim}

\paragraph{Mathematical Program}

\begin{align}
\max_{\allocvec} \,
& \sum_{i=1}^{\numbidders} \sum_{\val[i] \in \valspace[i]} f_i (\val[i]) \sqrt{\vvald[i]^+ (\val[i])} \sqrt{\hatalloc[i] (\val[i])} \\
\text{subject to }
%
& \sum_{i=1}^{n} f (\val[i]) \hatalloc[i] (\val[i]) \le 1
&& \\
%
& 0 \le \hatalloc[i] (\val[i]), 
&& \forall i \in \setofbidders, \forall \val[i] \in \valspace[i] \\
%
& \hatalloc[i] (\valz[i,\ell]) \ge \hatalloc[i] (\valz[i,\ell-1]), 
&& \forall i \in \setofbidders, \forall \valz[i,\ell] > \valz[i,\ell-1] \in \valspace[i] \\
\end{align}


\paragraph{Variables}

For each bidder $i \in \setofbidders$,
and for each $\val[i] \in \valspace[i]$, 
there are variables $\hatalloc[i] (\val[i])$.
The total number of variables is $O (nk)$.

\paragraph{Constraints}

The total number of constraints is $O(nk)$.  

\begin{itemize}
\item Ex-ante feasibility.  This requires $O(1)$ equations.
\item Lower bounds on $\hatalloc[i] (\val[i])$.  This requires $O(nk)$ equations.
\item Monotonicity.  This requires $O(nk)$ equations.
%\item Payment formula.  This requires $O(nk)$ equations.
\end{itemize}


==> programs/mpdesc_brm_xp_lb.tex <==

\subsubsection{BRM, Ex-post, Lower Bound (Heuristic)}
\label{sssec:mpdesc_brm_xp_lb}

\paragraph{Mathematical Program}

\begin{align}
\max_{\allocvec} \, 
& \sum_{i=1}^{n} \sum_{\val[i] \in \valspace[i]} f_i (\val[i]) \sqrt{\vvald[i]^+ (\val[i]) \hatalloc[i] (\val[i])} \\
\text{subject to }
%
& \sum_{i=1}^{n} \alloc[i] (\valvec) \le 1, 
&& \forall \valvec \in \valspace \\
%
& 0 \le \alloc[i] (\valvec), 
&& \forall i \in \setofbidders, \forall \valvec \in \valspace \\
%
& \alloc[i] (\valvec) \le 1, 
&& \forall i \in \setofbidders, \forall \valvec \in \valspace \\
%
& \hatalloc[i] (\val[i]) = \sum_{\valvec[-i]} f_{-i} (\valvec[-i]) \alloc[i] (\val[i], \valvec[-i]),
&& \forall i \in \setofbidders, \forall \val[i] \in \valspace[i] \\
%
& \hatalloc[i] (\valz[i,\ell]) \ge \hatalloc[i] (\valz[i,\ell-1]), 
&& \forall i \in \setofbidders, \forall \valz[i,\ell] > \valz[i,\ell-1] \in \valspace[i]
\end{align}

\paragraph{Variables}

For each bidder $i \in \setofbidders$ 
and for each $\val[i] \in \valspace[i]$
and $\valvec[-i] \in \valspace[-i]$, 
there are variables $\alloc[i] (\val[i], \valvec[-i])$.
%Additionally, there are variables $\hatalloc[i] (\val[i])$, for each $\val[i] \in \valspace[i]$.
The total number of variables is $O(n k^n)$.

\paragraph{Constraints}

The total number of constraints is $O(n k^n)$.  

\begin{itemize}
\item Ex-post feasibility.  This requires $O(k^n)$ equations.
\item Lower and upper bounds on $\alloc[i] (\val[i], \valvec[-i])$.  This requires $O(n k^n)$ equations.
\item Relating $\hatalloc[i] (\val[i])$ with $\alloc[i] (\val[i], \valvec[-i])$.  This requires $O (nk)$ equations.
\item Monotonicity.  This requires $O(n k)$ equations.
\end{itemize}


==> programs/mpdesc_brm_xp_lb_h.tex <==

\subsubsection{BRM, Ex-post, Lower Bound (Heuristic)}
\label{sssec:mpdesc_brm_xp_lb_h}

\commentt{This program describes the RRM lower bound.  This can be removed}

\paragraph{Mathematical Program}

\begin{align}
\max_{\allocvec} \, 
& \sum_{\valvec} \sum_{i=1}^{n} f (\valvec) \sqrt{\vvald[i]^+ (\val[i])} \sqrt{\alloc[i] (\valvec)} \\
\text{subject to }
%
& \sum_{i=1}^{n} \alloc[i] (\valvec) \le 1, 
&& \forall \valvec \in \valspace \\
%
& 0 \le \alloc[i] (\valvec), 
&& \forall i \in \setofbidders, \forall \valvec \in \valspace \\
%
& \alloc[i] (\valvec) \le 1, 
&& \forall i \in \setofbidders, \forall \valvec \in \valspace \\
%
& \alloc[i] (\valz[i,\ell], \valvec[-i]) \ge \alloc[i] (\valz[i,\ell-1], \valvec[-i]), 
&& \forall i \in \setofbidders, \forall \valz[i,\ell] > \valz[i,\ell-1] \in \valspace[i], \forall \valvec[-i] \in \valspace[-i]
\end{align}


\paragraph{Variables}

For each bidder $i \in \setofbidders$ 
and for each $\val[i] \in \valspace[i]$
and $\valvec[-i] \in \valspace[-i]$, 
there are variables $\alloc[i] (\val[i], \valvec[-i])$.
%Additionally, there are variables $\hatalloc[i] (\val[i])$, for each $\val[i] \in \valspace[i]$.
The total number of variables is $O(n k^n)$.

\paragraph{Constraints}

The total number of constraints is $O(n k^n)$.  

\begin{itemize}
\item Ex-post feasibility.  This requires $O(k^n)$ equations.
\item Lower and upper bounds on $\alloc[i] (\val[i], \valvec[-i])$.  This requires $O(n k^n)$ equations.
\item Monotonicity.  This requires $O(n k^n)$ equations.
%\item Relating $\hatalloc[i] (\val[i])$ with $\alloc[i] (\val[i], \valvec[-i])$.  This requires $O(nk)$ equations.
%\item Payment formula.  This requires $O(nk)$ equations.
\end{itemize}


==> results/bicFastSlowPayments.tex <==

\subsection{Bayesian Revenue Maximization}

We report the results of the following:
%
\begin{itemize}
\item (CPLEX) Total expected revenue of BRM XP without using Equation~\eqref{eq:hSquaredPayment}.  
(See Section~\ref{sssec:mpdesc_brm_xp_naive}.)
\item (CPLEX) Total expected revenue of BRM XP using Equation~\eqref{eq:hSquaredPayment}.
(See Section~\ref{sssec:mpdesc_brm_xp}.)
\end{itemize}
%
We see that when using Equation~\eqref{eq:hSquaredPayment}, we achieve
optimal total expected revenue, and solve the
%BRM, ex-post
problem more quickly.  This is to be expected, as the program
described in Section~\ref{sssec:mpdesc_brm_xp} has only
polynomially-many payment terms, and correspondingly fewer
constraints.

\begin{figure}[H]
    \centering
    \begin{subfigure}{.32\textwidth}
        \includegraphics[width=\textwidth]{figs/Categorical_brm_bef_aft_thm}
    \caption{Categorical Distribution}
\label{fig:catPlot_brmthm}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
    \includegraphics[width=\textwidth]{figs/Uniform_brm_bef_aft_thm}
    \caption{Uniform Distribution}
\label{fig:unifPlot_brmthm}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \includegraphics[width=\textwidth]{figs/Binomial_brm_bef_aft_thm}
    \caption{Binomial Distribution}
\label{fig:binomPlot_brmthm}
    \end{subfigure}
    \caption{BRM with and without Equation~\ref{eq:hSquaredPayment}}
\end{figure}



==> results/heuristic_bayesian.tex <==

\subsection{Heuristic Lower Bound and Heuristic Revenue in the Bayesian Problem}

We compare the heuristic lower bound in the robust problem
and the heuristic revenue in the Bayesian problem.
%
We report the results of the following two methods:
%
\begin{itemize}
\item (MATLAB) The heuristic lower bound in the robust problem
(see Section~\ref{sssec:mpdesc_rrm_xp_lb_h}) 
using Corollary~\ref{cor:rrm_ub_alloc_closedform} (the closed form).

\item (MATLAB) Heuristic revenue in the Bayesian problem:
First solve for the heuristic lower bound in the robust problem (see Section~\ref{sssec:mpdesc_rrm_xp_lb_h})
using Corollary~\ref{cor:rrm_ub_alloc_closedform} (the closed form);
then collapse the resulting allocations into interim allocations,
and use those to compute Bayesian payments
(Equation~\eqref{eq:hSquaredPayment}).
\end{itemize}

The heuristic lower bound and the heuristic revenue do not differ by
much.  Nor do the run times of the two methods; the heuristic lower
bound method does not calculate any payments at all, and the heuristic
revenue method calculates only polynomially many.

\begin{figure}[H]
    \centering
    \begin{subfigure}{.32\textwidth}
        \includegraphics[width=\textwidth]{figs/Categorical_brm_heurlb_heurrev}
    \caption{Categorical Distribution}
\label{fig:catPlot_brm_heurlb_heurrev}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
    \includegraphics[width=\textwidth]{figs/Uniform_brm_heurlb_heurrev}
    \caption{Uniform Distribution}
\label{fig:unifPlot_brm_heurlb_heurrev}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \includegraphics[width=\textwidth]{figs/Binomial_brm_heurlb_heurrev}
    \caption{Binomial Distribution}
\label{fig:binomPlot_brm_heurlb_heurrev}
    \end{subfigure}
    \caption{Heuristic Lower Bound and Heuristic Revenue in the Bayesian Problem}
\end{figure}

\commenta{interestingly, the run times of these methods do start to
increase quickly at around 20 bidders; but this could be a memory
issue. how do we figure out if this is an issue w/ swapping, as
opposed to an actual increase in the rate of increase of the run time?}


==> results/heuristic_robust.tex <==

\subsection{Heuristic Lower Bound and Heuristic Revenue in the Robust Problem}

We compare the heuristic lower bound and
the heuristic revenue in the robust problem.
%
We report the results of the following two methods:
%
\begin{itemize}
\item (MATLAB) The heuristic lower bound in the robust problem
(see Section~\ref{sssec:mpdesc_rrm_xp_lb_h}) 
using Corollary~\ref{cor:rrm_ub_alloc_closedform} (the closed form).

\item (MATLAB) Heuristic revenue in the robust problem:
First solve for the heuristic lower bound in the robust problem (see Section~\ref{sssec:mpdesc_rrm_xp_lb_h})
using Corollary~\ref{cor:rrm_ub_alloc_closedform} (the closed form);
then use the resulting allocations to compute robust payments (Equation~\eqref{eq:pSquaredPayment}).
\end{itemize}

The heuristic lower bound and the heuristic revenue do not differ by
much.  Their run times do differ however, since only the heuristic is
calculating payments.  But it seems that the heuristic lower bound
without computing payments yields a very quick, and remarkably
accurate, approximation.

\begin{figure}[H]
    \centering
    \begin{subfigure}{.32\textwidth}
        \includegraphics[width=\textwidth]{figs/Categorical_rrm_heurlb_heurrev}
    \caption{Categorical Distribution}
\label{fig:catPlot_rrm_heurlb_heurrev}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
    \includegraphics[width=\textwidth]{figs/Uniform_rrm_heurlb_heurrev}
    \caption{Uniform Distribution}
\label{fig:unifPlot_rrm_heurlb_heurrev}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \includegraphics[width=\textwidth]{figs/Binomial_rrm_heurlb_heurrev}
    \caption{Binomial Distribution}
\label{fig:binomPlot_rrm_heurlb_heurrev}
    \end{subfigure}
    \caption{Heuristic Lower Bound and Heuristic Revenue in the Robust Problem}
\end{figure}


